GrateTile: Efficient Sparse Tensor Tiling for CNN Processing

We propose GrateTile, an efficient, hardwarefriendly data storage scheme for sparse CNN feature maps (activations). It divides data into uneven-sized subtensors and, with small indexing overhead, stores them in a compressed yet randomly accessible format. This design enables modern CNN accelerators to fetch and decompressed sub-tensors on-the-fly in a tiled processing manner. GrateTile is suitable for architectures that favor aligned, coalesced data access, and only requires minimal changes to the overall architectural design. We simulate GrateTile with state-of-the-art CNNs and show an average of 55% DRAM bandwidth reduction while using only 0.6% of feature map size for indexing storage.

==> implementation.tex <==
\input{UMI_memex}

% MERIT is great for GPUs (SIMD)
% GPUs are not ideal SIMDs
% Use tiing to improve efficiency
Modern GPUs have SIMD-like designs that are suitable for workloads targeted by the MERIT transform.
However, because of the intricate design of GPU memory hierarchy, care must be taken while fetching data, as the latency introduced by cache misses tends to be fairly high.
Traditionally, in order to maximize data locality, programmers are responsible for dividing workloads into independent sub-tasks and plan the data fetches accordingly.
These very tedious \textit{tiling} or \textit{blocking} optimization processes can be replaced by factorized MERIT transforms, as shall be explained in the remainder of the section.

% Copied from ICCV
\subsection{Tiled Parallel Execution}
With the MERIT transform, supporting \textbf{t}iled execution can be simply achieved by dividing $M(\bA)$ and $M(\bB)$ into sub-tensors of sizes $(\bt_p, \bt_a)$.
\figref{merit_unr_shm} highlights some sub-tensors from \figref{merit_unrc} and \figref{merit_unrm}
with $(\bt_p, \bt_a) = ((2,2),(1,2))$ and $((2,2),(2))$, respectively.
It can be observed that for an arbitrary tensor $\bA$ and its transformed tensor $M(\bA)$,
each sub-tensor of $M(\bA)$ can be fully contained by a minimal sub-tensor of $\bA$, whose size at the $i$-th dimension is calculated by this equation
\begin{equation}\label{equ:footprint}
	1+\sum_j (t_j-1)s_j\delta_{d_j,i},
\end{equation}
where $d_j$ and $s_j$ represent the same axes and strides as in \equref{umi_um},
and $t_j$ denotes the size at the $j$-th dimension of the sub-tensor in the $M(\bA)$ domain.
This allows us to compute the memory footprint of the sub-tensor.
For example, using a $5$-by-$5$ kernel in convolution in order to obtain a $16$-by-$8$ pixel output,
we assign $(\bt_p, \bt_a)=((16, 8), (5,5))$ in \equref{footprint},
which gives the memory size requirement of $(1+1(16-1)+1(5-1), 1+1(8-1)+1(5-1)) = (20,12)$.
Instead of loading all elements of $M(\bA)$ directly from $\bA$, we first load its sub-tensor into user-addressable shared memory, and programmatically transform the tensor to the $M(\bA)$ domain on-the-fly, thereby eliminating all memory bandwidth overhead caused by duplication, since all data are load from the shared memory.

\subsection{Bank Conflict Avoidance}\label{sec:proc:bank_conflict}

% SRAM bank conflict what and why (same bank at the same time)
% bank conflict with MERIT
In GPUs, the shared memory may consist of many SRAM banks,
and the number of banks is usually designed to match the number of processor cores.
When the SIMD requests elements from the same SRAM at the same time,
the system performance drops drastically, causing the bank-conflict problem.
To avoid this problem, note that the vertical direction of the MERIT transformed matrices reflects the parallelism.
This property reduces bank-conflict problem into the analysis of column vector addresses within the sub-tensors of $M(\bA)$.

% Copied from ICCV
\figref{mex} illustrates examples for resolving bank-conflict
by padding~\cite[chap.~39]{gg3}, XOR-hash~\cite{xor1,xor2}, and our proposed \textit{re-tiling} technique.
The example shows a vector processor with 8 ALUs computing a $3\times 3$ convolution for a $4\times 4$ output block, requiring a $6\times 6$ block in total (\figref{mex}(i)).
The right parts of the figure illustrate some arrangements for distributing the $6\times 6$ pixel block into 8 SRAM banks physically.
In (ii-a), conflicts are highlighted in red,
whereas bank conflicts in (ii-b) are resolved by padding $6$ elements after every $6$ elements.
To reduce the padding waste, (ii-c) uses only $2$ padding with XOR-hash,
achieved by swapping the first and last four elements in every other row.
(iii) and (iv) show two different re-tiling that can create conflict-free scenarios without any hashing or padding requirement.
Later in \secref{proc}, we shall provide more details on finding suitable configurations and for storing and transferring of SRAM data.
We will also discuss our open-source implementation of the MERIT transform on GPUs in more details in \secref{eva}.

